Completion for braided enriched monoidal categories

Monoidal categories enriched in a braided monoidal category $\mathcal{V}$ are classified by braided oplax monoidal functors from $\mathcal{V}$ to the Drinfeld centers of ordinary monoidal categories. In this article, we prove that this classifying functor is strongly monoidal if and only if the original $\mathcal{V}$-monoidal category is tensored over $\mathcal{V}$. We then define a completion operation which produces a tensored $\mathcal{V}$-monoidal category $\overline{\mathcal{C}}$ from an arbitrary $\mathcal{V}$-monoidal category $\mathcal{C}$, and we determine many equivalent conditions which imply $\mathcal{C}$ and $\overline{\mathcal{C}}$ are $\mathcal{V}$-monoidally equivalent. Since being tensored is a property of the underlying $\mathcal{V}$-category of a $\mathcal{V}$-monoidal category, we begin by studying the equivalence between (tensored) $\mathcal{V}$-categories and oplax (strong) $\mathcal{V}$-module categories respectively. We then define the completion operation for $\mathcal{V}$-categories, and adapt these results to the $\mathcal{V}$-monoidal setting.

==> tikzlibraryknots.code.tex <==
%%
%% This is file `tikzlibraryknots.code.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% spath3.dtx  (with options: `knots')
%% ----------------------------------------------------------------
%% spath3 --- Functions for manipulating PGF soft paths
%% E-mail: stacey@math.ntnu.no
%% Released under the LaTeX Project Public License v1.3c or later
%% See http://www.latex-project.org/lppl.txt
%% ----------------------------------------------------------------
%% 
%%
\RequirePackage{spath3}
\usetikzlibrary{intersections}

\ExplSyntaxOn

\tl_new:N \l__knot_tmpa_tl
\tl_new:N \l__knot_tmpb_tl
\tl_new:N \l__knot_tmpc_tl
\tl_new:N \l__knot_tmpd_tl
\tl_new:N \l__knot_tmpe_tl
\tl_new:N \l__knot_tmpf_tl
\tl_new:N \l__knot_tmpg_tl
\tl_new:N \l__knot_redraws_tl
\tl_new:N \l__knot_clip_width_tl
\tl_new:N \l__knot_name_tl
\tl_new:N \l__knot_node_tl

\int_new:N \l__knot_tmpa_int
\int_new:N \l__knot_strands_int
\int_new:N \l__knot_intersections_int
\int_new:N \l__knot_filaments_int
\int_new:N \l__knot_component_start_int

\dim_new:N \l__knot_tmpa_dim
\dim_new:N \l__knot_tmpb_dim
\dim_new:N \l__knot_tmpc_dim
\dim_new:N \l__knot_tolerance_dim
\dim_new:N \l__knot_clip_radius_dim

\bool_new:N \l__knot_draft_bool
\bool_new:N \l__knot_ignore_ends_bool
\bool_new:N \l__knot_self_intersections_bool
\bool_new:N \l__knot_splits_bool
\bool_new:N \l__knot_super_draft_bool

\bool_new:N \l__knot_prepend_prev_bool
\bool_new:N \l__knot_append_next_bool
\bool_new:N \l__knot_skip_bool

\bool_set_true:N \l__knot_ignore_ends_bool
\tikzset{
  knot/.code={
    \tl_if_eq:nnTF {#1} {none}
    {
      \tikz@addmode{\tikz@mode@doublefalse}
    }
    {
      \tikz@addmode{\tikz@mode@doubletrue}
      \tl_if_eq:nnTF {\pgfkeysnovalue} {#1}
      {
        \tikz@addoption{\pgfsetinnerstrokecolor{.}}
      }
      {
        \pgfsetinnerstrokecolor{#1}
      }
      \tikz@addoption{
        \pgfsetstrokecolor{knotbg}
      }
      \tl_set:Nn \tikz@double@setup{
        \pgfsetinnerlinewidth{\pgflinewidth}
        \pgfsetlinewidth{\dim_eval:n {\tl_use:N \l__knot_gap_tl \pgflinewidth}}
      }
    }
  },
  knot~ gap/.store~ in=\l__knot_gap_tl,
  knot~ gap=3,
  knot~ diagram/.is~family,
  knot~ diagram/.unknown/.code={
    \tl_set_eq:NN \l__knot_tmpa_tl \pgfkeyscurrentname
    \pgfkeysalso{
      /tikz/\l__knot_tmpa_tl=#1
    }
  },
  background~ colour/.code={%
    \colorlet{knotbg}{#1}%
  },
  background~ color/.code={%
    \colorlet{knotbg}{#1}%
  },
  background~ colour=white,
  knot~ diagram,
  name/.store~in=\l__knot_name_tl,
  name={knot},
  every~ strand/.style={draw},
  ignore~ endpoint~ intersections/.code={
    \tl_if_eq:nnTF {#1} {true}
    {
      \bool_set_true:N \l__knot_ignore_ends_bool
    }
    {
      \bool_set_false:N \l__knot_ignore_ends_bool
    }
  },
  ignore~ endpoint~ intersections/.default=true,
  consider~ self~ intersections/.is~choice,
  consider~ self~ intersections/true/.code={
    \bool_set_true:N \l__knot_self_intersections_bool
    \bool_set_true:N \l__knot_splits_bool
  },
  consider~ self~ intersections/false/.code={
    \bool_set_false:N \l__knot_self_intersections_bool
    \bool_set_false:N \l__knot_splits_bool
  },
  consider~ self~ intersections/no~ splits/.code={
    \bool_set_true:N \l__knot_self_intersections_bool
    \bool_set_false:N \l__knot_splits_bool
  },
  consider~ self~ intersections/.default={true},
  clip~ radius/.code={
    \dim_set:Nn \l__knot_clip_radius_dim {#1}
  },
  clip~ radius=10pt,
  end~ tolerance/.code={
    \dim_set:Nn \l__knot_tolerance_dim {#1}
  },
  end~ tolerance=14pt,
  clip~ width/.code={
    \tl_set:Nn \l__knot_clip_width_tl {#1}
  },
  clip~ width=3,
  flip~ crossing/.code={%
    \tl_clear_new:c {l__knot_crossing_#1}
    \tl_set:cn {l__knot_crossing_#1} {x}
  },
  draft~ mode/.is~ choice,
  draft~ mode/off/.code={%
    \bool_set_false:N \l__knot_draft_bool
    \bool_set_false:N \l__knot_super_draft_bool
  },
  draft~ mode/crossings/.code={%
    \bool_set_true:N \l__knot_draft_bool
    \bool_set_false:N \l__knot_super_draft_bool
  },
  draft~ mode/strands/.code={%
    \bool_set_true:N \l__knot_draft_bool
    \bool_set_true:N \l__knot_super_draft_bool
  },
  draft/.is~ family,
  draft,
  crossing~ label/.style={
    overlay,
    fill=white,
    fill~ opacity=.5,
    text~ opacity=1,
    text=blue,
    pin~ edge={blue,<-}
  },
  strand~ label/.style={
    overlay,
    circle,
    draw=purple,
    fill=white,
    fill~ opacity=.5,
    text~ opacity=1,
    text=purple,
    inner~ sep=0pt
  },
}
\cs_new_nopar:Npn \knot_apply_style:N #1
{
  \tl_if_exist:NT #1 {
    \exp_args:NV \tikzset #1
  }
}
\cs_generate_variant:Nn \knot_apply_style:N {c}
\NewDocumentCommand \flipcrossings {m}
{
  \tikzset{knot~ diagram/flip~ crossing/.list={#1}}%
}
\NewDocumentCommand \strand { O{} }
{
  \int_incr:N \l__knot_strands_int
  \tl_clear_new:c {l__knot_options_strand \int_use:N \l__knot_strands_int}
  \tl_set:cn {l__knot_options_strand \int_use:N \l__knot_strands_int} {#1}
  \path[#1,save~ spath=knot strand \int_use:N  \l__knot_strands_int]
}
\NewDocumentEnvironment{knot} { O{} }
{
  \knot_initialise:n {#1}
}
{
  \knot_render:
}
\cs_new_protected_nopar:Npn \knot_initialise:n #1
{
  \tikzset{knot~ diagram/.cd,every~ knot~ diagram/.try,#1}
  \int_zero:N \l__knot_strands_int
  \tl_clear:N \l__knot_redraws_tl
}
\cs_new_protected_nopar:Npn \knot_render:
{
  \pgfscope
  \pgftransformreset
  \int_step_function:nnnN {1} {1} {\l__knot_strands_int} \knot_draw_strand:n
  \bool_if:NF \l__knot_super_draft_bool
  {
    \int_step_function:nnnN {1} {1} {\l__knot_strands_int} \knot_draw_labels:n
    \bool_if:NTF \l__knot_self_intersections_bool
    {
      \knot_split_strands:
      \int_set_eq:NN \l__knot_tmpa_int \l__knot_filaments_int
      \tl_set:Nn \l__knot_prefix_tl {filament}
    }
    {
      \int_set_eq:NN \l__knot_tmpa_int \l__knot_strands_int
      \tl_set:Nn \l__knot_prefix_tl {strand}
    }
    \int_gzero:N \l__knot_intersections_int
    \bool_if:NTF \l__knot_draft_bool
    {
      \tl_set:Nn \l__knot_node_tl
      {\node[coordinate,pin={[knot~ diagram/draft/crossing~ label]{\int_use:N \l__knot_intersections_int}}]}
    }
    {
      \tl_set:Nn \l__knot_node_tl {\node[coordinate]}
    }
    \int_step_variable:nnnNn {1} {1} {\l__knot_tmpa_int - 1} \l__knot_tmpa_tl
    {
      \int_step_variable:nnnNn {\tl_use:N \l__knot_tmpa_tl + 1} {1}     {\l__knot_tmpa_int} \l__knot_tmpb_tl
      {
        \knot_intersections:VV \l__knot_tmpa_tl \l__knot_tmpb_tl
      }
    }
    \tl_use:N \l__knot_redraws_tl
  }
  \endpgfscope
}
\cs_new_protected_nopar:Npn \knot_draw_strand:n #1
{
  \pgfscope
  \group_begin:
  \tl_set:Nn \l_tmpa_tl {knot~ diagram/every~ strand/.try,}
  \tl_put_right:Nv \l_tmpa_tl {l__knot_options_strand #1}
  \tl_put_right:Nn \l_tmpa_tl {,knot~ diagram/only~ when~ rendering/.try,only~ when~ rendering/.try}
  \spath_bake_round:n {knot strand #1}
  \spath_tikz_path:Vn \l_tmpa_tl {knot strand #1}
  \group_end:
  \endpgfscope
}
\cs_generate_variant:Nn \tl_put_right:Nn {Nv}
\cs_new_protected_nopar:Npn \knot_draw_labels:n #1
{
  \bool_if:NT \l__knot_draft_bool
  {
    \spath_get:nnN {knot strand #1} {final point} \l__knot_tmpb_tl
    \dim_set:Nn \l__knot_tmpa_dim {\tl_item:Nn \l__knot_tmpb_tl {1}}
    \dim_set:Nn \l__knot_tmpb_dim {\tl_item:Nn \l__knot_tmpb_tl {2}}
    \node[knot~ diagram/draft/strand~label] at (\l__knot_tmpa_dim,\l__knot_tmpb_dim) {#1};
    \spath_get:nnN {knot strand #1} {initial point} \l__knot_tmpb_tl
    \dim_set:Nn \l__knot_tmpa_dim {\tl_item:Nn \l__knot_tmpb_tl {1}}
    \dim_set:Nn \l__knot_tmpb_dim {\tl_item:Nn \l__knot_tmpb_tl {2}}
    \node[knot~ diagram/draft/strand~label] at (\l__knot_tmpa_dim,\l__knot_tmpb_dim) {#1};
  }
  \bool_if:nT {
    \l__knot_self_intersections_bool
    &&
    \l__knot_splits_bool
  }
  {
    \tl_clear:N \l__knot_tmpa_tl
    \spath_map_segment_function:nN {knot strand #1} \knot_split_self_intersects:NN
    \spath_put:nnV {knot strand #1} {path} \l__knot_tmpa_tl
  }
}
\cs_new_protected_nopar:Npn \knot_split_self_intersects:NN #1#2
{
  \tl_case:NnF #1
  {
    \g__spath_curvetoa_tl
    {
      \fp_set:Nn \l_tmpa_fp
      {
        (\tl_item:Nn #2 {3} - 3 * \tl_item:Nn #2 {6} + 3 * \tl_item:Nn #2 {9} - \tl_item:Nn #2 {12})
        *
        (3 * \tl_item:Nn #2 {8} - 3 * \tl_item:Nn #2 {11})
        -
        (\tl_item:Nn #2 {2} - 3 * \tl_item:Nn #2 {5} + 3 * \tl_item:Nn #2 {8} - \tl_item:Nn #2 {11})
        *
        (3 * \tl_item:Nn #2 {9} - 3 * \tl_item:Nn #2 {12})
      }
      \fp_set:Nn \l_tmpb_fp
      {
        (\tl_item:Nn #2 {2} - 3 * \tl_item:Nn #2 {5} + 3 * \tl_item:Nn #2 {8} - \tl_item:Nn #2 {11})
        *
        (3 * \tl_item:Nn #2 {6} - 6 * \tl_item:Nn #2 {9} + 3 * \tl_item:Nn #2 {12})
        -
        (\tl_item:Nn #2 {3} - 3 * \tl_item:Nn #2 {6} + 3 * \tl_item:Nn #2 {9} - \tl_item:Nn #2 {12})
        *
        (3 * \tl_item:Nn #2 {5} - 6 * \tl_item:Nn #2 {8} + 3 * \tl_item:Nn #2 {11})
      }
      \fp_compare:nTF
      {
        \l_tmpb_fp != 0
      }
      {
        \fp_set:Nn \l_tmpa_fp {.5 * \l_tmpa_fp / \l_tmpb_fp}
        \fp_compare:nTF
        {
          0 < \l_tmpa_fp && \l_tmpa_fp < 1
        }
        {
          \spath_split_curve:VVNN \l_tmpa_fp #2 \l_tmpa_tl \l_tmpb_tl
          \tl_set:Nx \l_tmpa_tl {\tl_tail:N \l_tmpa_tl}
          \tl_set:Nx \l_tmpa_tl {\tl_tail:N \l_tmpa_tl}
          \tl_set:Nx \l_tmpa_tl {\tl_tail:N \l_tmpa_tl}
          \tl_set:Nx \l_tmpb_tl {\tl_tail:N \l_tmpb_tl}
          \tl_set:Nx \l_tmpb_tl {\tl_tail:N \l_tmpb_tl}
          \tl_set:Nx \l_tmpb_tl {\tl_tail:N \l_tmpb_tl}
          \tl_put_right:NV \l__knot_tmpa_tl \l_tmpa_tl
          \tl_put_right:NV \l__knot_tmpa_tl \l_tmpb_tl
        }
        {
          \tl_set_eq:NN \l_tmpa_tl #2
          \tl_set:Nx \l_tmpa_tl {\tl_tail:N \l_tmpa_tl}
          \tl_set:Nx \l_tmpa_tl {\tl_tail:N \l_tmpa_tl}
          \tl_set:Nx \l_tmpa_tl {\tl_tail:N \l_tmpa_tl}
          \tl_put_right:NV \l__knot_tmpa_tl \l_tmpa_tl
        }
      }
      {
        \tl_set_eq:NN \l_tmpa_tl #2
        \tl_set:Nx \l_tmpa_tl {\tl_tail:N \l_tmpa_tl}
        \tl_set:Nx \l_tmpa_tl {\tl_tail:N \l_tmpa_tl}
        \tl_set:Nx \l_tmpa_tl {\tl_tail:N \l_tmpa_tl}
        \tl_put_right:NV \l__knot_tmpa_tl \l_tmpa_tl
      }
    }
    \g__spath_lineto_tl
    {
      \tl_set_eq:NN \l_tmpa_tl #2
      \tl_set:Nx \l_tmpa_tl {\tl_tail:N \l_tmpa_tl}
      \tl_set:Nx \l_tmpa_tl {\tl_tail:N \l_tmpa_tl}
      \tl_set:Nx \l_tmpa_tl {\tl_tail:N \l_tmpa_tl}
      \tl_put_right:NV \l__knot_tmpa_tl \l_tmpa_tl
    }
  }
  {
    \tl_put_right:NV \l__knot_tmpa_tl #2
  }
}
\cs_new_protected_nopar:Npn \knot_intersections:nn #1#2
{
  \group_begin:
  \tl_set_eq:NN \l__knot_tmpa_tl \l__knot_prefix_tl
  \tl_put_right:Nn \l__knot_tmpa_tl {#1}
  \tl_set_eq:NN \l__knot_tmpb_tl \l__knot_prefix_tl
  \tl_put_right:Nn \l__knot_tmpb_tl {#2}
  \spath_get:nnN {knot \tl_use:N \l__knot_tmpa_tl} {path} \l__knot_tmpc_tl
  \spath_get:nnN {knot \tl_use:N \l__knot_tmpb_tl} {path} \l__knot_tmpd_tl

  \pgfintersectionofpaths{\pgfsetpath\l__knot_tmpc_tl}{\pgfsetpath\l__knot_tmpd_tl}

  \int_compare:nT {\pgfintersectionsolutions > 0}
  {
    \int_step_function:nnnN {1} {1} {\pgfintersectionsolutions} \knot_do_intersection:n
  }
  \group_end:
}
\cs_new_protected_nopar:Npn \knot_do_intersection:n #1
{
  \pgfpointintersectionsolution{#1}
  \dim_set:Nn \l__knot_tmpa_dim {\pgf@x}
  \dim_set:Nn \l__knot_tmpb_dim {\pgf@y}
  \bool_set_false:N \l__knot_skip_bool
  \bool_if:NT \l__knot_self_intersections_bool
  {
    \tl_set:Nn \l_tmpa_tl {knot previous}
    \tl_put_right:NV \l_tmpa_tl \l__knot_tmpa_tl
    \tl_set:Nv \l_tmpa_tl \l_tmpa_tl
    \tl_if_eq:NNT \l_tmpa_tl \l__knot_tmpb_tl
    {
      \knot_test_endpoint:VnT \l__knot_tmpb_tl {final point}
      {
        \bool_set_true:N \l__knot_skip_bool
      }
    }

    \tl_set:Nn \l_tmpa_tl {knot previous}
    \tl_put_right:NV \l_tmpa_tl \l__knot_tmpb_tl
    \tl_set:Nv \l_tmpa_tl \l_tmpa_tl
    \tl_if_eq:NNT \l_tmpa_tl \l__knot_tmpa_tl
    {
      \knot_test_endpoint:VnT \l__knot_tmpa_tl {final point}
      {
        \bool_set_true:N \l__knot_skip_bool
      }
    }
  }
  \bool_if:NT \l__knot_ignore_ends_bool
  {
    \knot_test_endpoint:VnT \l__knot_tmpa_tl {initial point}
    {
      \bool_set_true:N \l__knot_skip_bool
    }
    \knot_test_endpoint:VnT \l__knot_tmpa_tl {final point}
    {
      \bool_set_true:N \l__knot_skip_bool
    }
    \knot_test_endpoint:VnT \l__knot_tmpb_tl {initial point}
    {
      \bool_set_true:N \l__knot_skip_bool
    }
    \knot_test_endpoint:VnT \l__knot_tmpb_tl {final point}
    {
      \bool_set_true:N \l__knot_skip_bool
    }
  }
  \bool_if:NF \l__knot_skip_bool
  {

    \int_gincr:N \l__knot_intersections_int
    \bool_if:nTF
    {
      \tl_if_exist_p:c {l__knot_crossing_ \int_use:N
        \l__knot_intersections_int}
      &&
      ! \tl_if_empty_p:c {l__knot_crossing_ \int_use:N
        \l__knot_intersections_int}
    }
    {
      \tl_set_eq:NN \l__knot_tmpg_tl \l__knot_tmpb_tl
    }
    {
      \tl_set_eq:NN \l__knot_tmpg_tl \l__knot_tmpa_tl
    }
    \bool_if:NT \l__knot_self_intersections_bool
    {
      \knot_test_endpoint:VnT \l__knot_tmpg_tl {initial point}
      {
        \bool_set_true:N \l__knot_prepend_prev_bool
      }
      {
        \bool_set_false:N \l__knot_prepend_prev_bool
      }

      \knot_test_endpoint:VnT \l__knot_tmpg_tl {final point}
      {
        \bool_set_true:N \l__knot_append_next_bool
      }
      {
        \bool_set_false:N \l__knot_append_next_bool
      }
      \bool_if:nT
      {
        \l__knot_prepend_prev_bool || \l__knot_append_next_bool
      }
      {
        \spath_clone:nn {knot \tl_use:N \l__knot_tmpg_tl}
        {knot \tl_use:N \l__knot_prefix_tl -1}

        \tl_set_eq:cc {l__knot_options_ \tl_use:N \l__knot_prefix_tl -1} {l__knot_options_ \tl_use:N \l__knot_tmpg_tl}

        \bool_if:nT
        {
          \l__knot_prepend_prev_bool
          &&
          \tl_if_exist_p:c {knot previous \tl_use:N \l__knot_tmpg_tl}
          &&
          !\tl_if_empty_p:c {knot previous \tl_use:N \l__knot_tmpg_tl}
        }
        {
          \spath_prepend_no_move:nn {knot \tl_use:N \l__knot_prefix_tl -1} {knot \tl_use:c {knot previous \tl_use:N \l__knot_tmpg_tl}}
          \bool_if:nT
          {
            \l__knot_splits_bool
            &&
            \tl_if_exist_p:c {knot previous \tl_use:N \l__knot_tmpg_tl}
            &&
            !\tl_if_empty_p:c {knot previous \tl_use:N \l__knot_tmpg_tl}
          }
          {
            \knot_test_endpoint:vnT {knot previous \tl_use:N \l__knot_tmpg_tl} {initial point}
            {
              \spath_get:nnN {knot \tl_use:N \l__knot_prefix_tl -1} {path} \l_tmpa_tl
              \spath_prepend_no_move:nn {knot \tl_use:N \l__knot_prefix_tl -1} {knot \tl_use:c {knot previous \tl_use:c {knot previous \tl_use:N \l__knot_tmpg_tl}}}
              \spath_get:nnN {knot \tl_use:N \l__knot_prefix_tl -1} {path} \l_tmpa_tl

            }
          }
        }
        \bool_if:nT
        {
          \l__knot_append_next_bool
          &&
          \tl_if_exist_p:c {knot next \tl_use:N \l__knot_tmpg_tl}
          &&
          !\tl_if_empty_p:c {knot previous \tl_use:N \l__knot_tmpg_tl}
        }
        {
          \spath_append_no_move:nn {knot \tl_use:N \l__knot_prefix_tl -1} {knot \tl_use:c {knot next \tl_use:N \l__knot_tmpg_tl}}
          \bool_if:nT
          {
            \l__knot_splits_bool
            &&
            \tl_if_exist_p:c {knot previous \tl_use:N
              \l__knot_tmpg_tl}
            &&
            !\tl_if_empty_p:c {knot previous \tl_use:N \l__knot_tmpg_tl}
          }
          {
            \knot_test_endpoint:vnT {knot previous \tl_use:N \l__knot_tmpg_tl} {final point}
            {
              \spath_append_no_move:nn {knot \tl_use:N \l__knot_prefix_tl -1} {knot \tl_use:c {knot next \tl_use:c {knot next \tl_use:N \l__knot_tmpg_tl}}}

            }
          }
        }

        \tl_set:Nn \l__knot_tmpg_tl {\tl_use:N \l__knot_prefix_tl -1}
      }
    }
    \pgfscope
    \group_begin:
    \tikzset{knot~ diagram/every~ intersection/.try, every~ intersection/.try, knot~ diagram/intersection~ \int_use:N \l__knot_intersections_int/.try}
    \knot_draw_crossing:nVV {\tl_use:N \l__knot_tmpg_tl} \l__knot_tmpa_dim \l__knot_tmpb_dim
    \group_end:
    \endpgfscope
    \tl_use:N \l__knot_node_tl (\l__knot_name_tl \c_space_tl \int_use:N \l__knot_intersections_int) at (\l__knot_tmpa_dim, \l__knot_tmpb_dim) {};
  }
}

\cs_generate_variant:Nn \knot_intersections:nn {VV}
\prg_new_conditional:Npnn \knot_test_endpoint:N #1 {p,T,F,TF}
{
  \dim_compare:nTF
  {
    \dim_abs:n {\pgf@x - \tl_item:Nn #1 {1}}
    +
    \dim_abs:n {\pgf@y - \tl_item:Nn #1 {2}}
    <
    \l__knot_tolerance_dim
  }
  {
    \prg_return_true:
  }
  {
    \prg_return_false:
  }
}
\prg_new_protected_conditional:Npnn \knot_test_endpoint:nn #1#2 {T,F,TF}
{
  \spath_get:nnN {knot #1} {#2} \l__knot_tmpd_tl
  \knot_test_endpoint:NTF \l__knot_tmpd_tl
  {
    \prg_return_true:
  }
  {
    \prg_return_false:
  }
}

\cs_generate_variant:Nn \knot_test_endpoint:nnT {VnT,vnT}
\cs_generate_variant:Nn \knot_test_endpoint:nnF {VnF,vnF}
\cs_generate_variant:Nn \knot_test_endpoint:nnTF {VnTF,vnTF}
\cs_new_nopar:Npn \knot_draw_crossing:nnn #1#2#3
{
  \group_begin:
  \pgfscope
  \clip (#2, #3) circle[radius=\l__knot_clip_radius_dim];

  \tl_set:Nn \l_tmpa_tl {knot~ diagram/every~ strand/.try,}
  \tl_if_exist:cT {l__knot_options_ #1}
  {
  \tl_put_right:Nv \l_tmpa_tl {l__knot_options_ #1}
  }
  \tl_put_right:Nn \l_tmpa_tl {,knotbg,line~ width= \tl_use:N \l__knot_clip_width_tl * \pgflinewidth}
  \spath_tikz_path:Vn \l_tmpa_tl {knot #1}

  \endpgfscope

  \pgfscope
  \clip (#2, #3) circle[radius=1.1\l__knot_clip_radius_dim];

  \tl_set:Nn \l_tmpa_tl {knot~ diagram/every~ strand/.try,}
  \tl_if_exist:cT {l__knot_options_ #1}
  {
  \tl_put_right:Nv \l_tmpa_tl {l__knot_options_ #1}
  }
  \tl_put_right:Nn \l_tmpa_tl {,knot~ diagram/only~ when~ rendering/.try,only~ when~ rendering/.try}
  \spath_tikz_path:Vn \l_tmpa_tl {knot #1}

  \endpgfscope
  \group_end:
}

\cs_generate_variant:Nn \knot_draw_crossing:nnn {nVV}
\cs_new_protected_nopar:Npn \knot_split_strands:
{
  \int_gzero:N \l__knot_filaments_int
  \int_step_function:nnnN {1} {1} {\l__knot_strands_int} \knot_split_strand:n
  \int_step_function:nnnN {1} {1} {\l__knot_filaments_int} \knot_compute_nexts:n
}
\cs_new_protected_nopar:Npn \knot_compute_nexts:n #1
{
  \tl_clear_new:c {knot next \tl_use:c {knot previous filament #1}}
  \tl_set:cn {knot next \tl_use:c {knot previous filament #1}} {filament #1}
}
\cs_new_protected_nopar:Npn \knot_split_strand:n #1
{
  \int_set_eq:NN \l__knot_component_start_int \l__knot_filaments_int
  \int_incr:N \l__knot_component_start_int
  \tl_set_eq:Nc \l__knot_tmpa_tl {l__knot_options_strand #1}
  \spath_map_segment_function:nN {knot strand #1} \knot_save_filament:NN
}
\cs_new_protected_nopar:Npn \knot_save_filament:NN #1#2
{
  \tl_case:NnF #1
  {
    \g__spath_moveto_tl
    {
      \int_compare:nT {\l__knot_component_start_int < \l__knot_filaments_int}
      {
        \int_set_eq:NN \l__knot_component_start_int \l__knot_filaments_int
      }
    }
    \g__spath_lineto_tl
    {
      \int_gincr:N \l__knot_filaments_int
      \spath_clear_new:n {knot filament \int_use:N \l__knot_filaments_int}
      \spath_put:nnV {knot filament \int_use:N \l__knot_filaments_int} {path} #2
      \tl_set_eq:cN {l__knot_options_filament \int_use:N \l__knot_filaments_int} \l__knot_tmpa_tl

      \tl_clear_new:c {knot previous filament \int_use:N \l__knot_filaments_int}
      \int_compare:nF {\l__knot_component_start_int == \l__knot_filaments_int}
      {
        \tl_set:cx {knot previous filament \int_use:N \l__knot_filaments_int} {filament \int_eval:n {\l__knot_filaments_int - 1}}
      }
    }
    \g__spath_curvetoa_tl
    {
      \int_gincr:N \l__knot_filaments_int
      \spath_clear_new:n {knot filament \int_use:N \l__knot_filaments_int}
      \spath_put:nnV {knot filament \int_use:N \l__knot_filaments_int} {path} #2
      \tl_set_eq:cN {l__knot_options_filament \int_use:N \l__knot_filaments_int} \l__knot_tmpa_tl

      \tl_clear_new:c {knot previous filament \int_use:N \l__knot_filaments_int}
      \int_compare:nF {\l__knot_component_start_int == \l__knot_filaments_int}
      {
        \tl_set:cx {knot previous filament \int_use:N \l__knot_filaments_int} {filament \int_eval:n {\l__knot_filaments_int - 1}}
      }
    }
    \g__spath_close_tl
    {
      \int_gincr:N \l__knot_filaments_int
      \spath_clear_new:n {knot filament \int_use:N \l__knot_filaments_int}
      \tl_set_eq:NN \l_tmpa_tl #2
      \tl_set:Nx \l_tmpa_tl {\tl_item:Nn #2 {1}\tl_item:Nn #2 {2}\tl_item:Nn #2 {3}}
      \tl_put_right:NV \l_tmpa_tl \g__spath_lineto_tl
      \tl_set:Nx \l_tmpa_tl {\tl_item:Nn #2 {5}\tl_item:Nn #2 {6}}
      \spath_put:nnV {knot filament \int_use:N \l__knot_filaments_int} {path} \l_tmpa_tl
      \tl_set_eq:cN {l__knot_options_filament \int_use:N \l__knot_filaments_int} \l__knot_tmpa_tl
      \tl_clear_new:c {knot previous filament \int_use:N \l__knot_filaments_int}
      \int_compare:nF {\l__knot_component_start_int == \l__knot_filaments_int}
      {
        \tl_set:cx {knot previous filament \int_use:N \l__knot_filaments_int} {filament \int_eval:n {\l__knot_filaments_int - 1}}
      }
      \tl_set:cx {knot previous filament \int_use:N \l__knot_component_start_int} {filament \int_use:N \l__knot_filaments_int}
    }
  }
  {
  }
}
\NewDocumentCommand \redraw { m m }
{
  \tikz@scan@one@point\pgfutil@firstofone #2 \relax
  \tl_put_right:Nn \l__knot_redraws_tl {\knot_draw_crossing:nnn}
  \tl_put_right:Nx \l__knot_redraws_tl {
    {strand #1} {\dim_use:N \pgf@x} {\dim_use:N \pgf@y}
  }
}
\ExplSyntaxOff
\def\pgf@sh@@knotanchor#1#2{%
  \anchor{#2 north west}{%
    \csname pgf@anchor@knot #1@north west\endcsname%
    \pgf@x=#2\pgf@x%
    \pgf@y=#2\pgf@y%
  }%
  \anchor{#2 north east}{%
    \csname pgf@anchor@knot #1@north east\endcsname%
    \pgf@x=#2\pgf@x%
    \pgf@y=#2\pgf@y%
  }%
  \anchor{#2 south west}{%
    \csname pgf@anchor@knot #1@south west\endcsname%
    \pgf@x=#2\pgf@x%
    \pgf@y=#2\pgf@y%
  }%
  \anchor{#2 south east}{%
    \csname pgf@anchor@knot #1@south east\endcsname%
    \pgf@x=#2\pgf@x%
    \pgf@y=#2\pgf@y%
  }%
  \anchor{#2 north}{%
    \csname pgf@anchor@knot #1@north\endcsname%
    \pgf@x=#2\pgf@x%
    \pgf@y=#2\pgf@y%
  }%
  \anchor{#2 east}{%
    \csname pgf@anchor@knot #1@east\endcsname%
    \pgf@x=#2\pgf@x%
    \pgf@y=#2\pgf@y%
  }%
  \anchor{#2 west}{%
    \csname pgf@anchor@knot #1@west\endcsname%
    \pgf@x=#2\pgf@x%
    \pgf@y=#2\pgf@y%
  }%
  \anchor{#2 south}{%
    \csname pgf@anchor@knot #1@south\endcsname%
    \pgf@x=#2\pgf@x%
    \pgf@y=#2\pgf@y%
  }%
}
\pgfdeclareshape{knot crossing}
{
  \inheritsavedanchors[from=circle] % this is nearly a circle
  \inheritanchorborder[from=circle]
  \inheritanchor[from=circle]{north}
  \inheritanchor[from=circle]{north west}
  \inheritanchor[from=circle]{north east}
  \inheritanchor[from=circle]{center}
  \inheritanchor[from=circle]{west}
  \inheritanchor[from=circle]{east}
  \inheritanchor[from=circle]{mid}
  \inheritanchor[from=circle]{mid west}
  \inheritanchor[from=circle]{mid east}
  \inheritanchor[from=circle]{base}
  \inheritanchor[from=circle]{base west}
  \inheritanchor[from=circle]{base east}
  \inheritanchor[from=circle]{south}
  \inheritanchor[from=circle]{south west}
  \inheritanchor[from=circle]{south east}
  \inheritanchorborder[from=circle]
  \pgf@sh@@knotanchor{crossing}{2}
  \pgf@sh@@knotanchor{crossing}{3}
  \pgf@sh@@knotanchor{crossing}{4}
  \pgf@sh@@knotanchor{crossing}{8}
  \pgf@sh@@knotanchor{crossing}{16}
  \pgf@sh@@knotanchor{crossing}{32}
  \backgroundpath{
    \pgfutil@tempdima=\radius%
    \pgfmathsetlength{\pgf@xb}{\pgfkeysvalueof{/pgf/outer xsep}}%
    \pgfmathsetlength{\pgf@yb}{\pgfkeysvalueof{/pgf/outer ysep}}%
    \ifdim\pgf@xb<\pgf@yb%
      \advance\pgfutil@tempdima by-\pgf@yb%
    \else%
      \advance\pgfutil@tempdima by-\pgf@xb%
    \fi%
  }
}
\pgfdeclareshape{knot over cross}
{
  \inheritsavedanchors[from=rectangle] % this is nearly a circle
  \inheritanchorborder[from=rectangle]
  \inheritanchor[from=rectangle]{north}
  \inheritanchor[from=rectangle]{north west}
  \inheritanchor[from=rectangle]{north east}
  \inheritanchor[from=rectangle]{center}
  \inheritanchor[from=rectangle]{west}
  \inheritanchor[from=rectangle]{east}
  \inheritanchor[from=rectangle]{mid}
  \inheritanchor[from=rectangle]{mid west}
  \inheritanchor[from=rectangle]{mid east}
  \inheritanchor[from=rectangle]{base}
  \inheritanchor[from=rectangle]{base west}
  \inheritanchor[from=rectangle]{base east}
  \inheritanchor[from=rectangle]{south}
  \inheritanchor[from=rectangle]{south west}
  \inheritanchor[from=rectangle]{south east}
  \inheritanchorborder[from=rectangle]
  \backgroundpath{
    \southwest \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgfpathmoveto{\pgfqpoint{\pgf@xa}{\pgf@ya}}
    \pgfpathlineto{\pgfqpoint{\pgf@xb}{\pgf@yb}}
  }
  \foregroundpath{
    \southwest \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgfpathmoveto{\pgfqpoint{\pgf@xa}{\pgf@yb}}
    \pgfpathlineto{\pgfqpoint{\pgf@xb}{\pgf@ya}}
 }
}
\pgfdeclareshape{knot under cross}
{
  \inheritsavedanchors[from=rectangle] % this is nearly a circle
  \inheritanchorborder[from=rectangle]
  \inheritanchor[from=rectangle]{north}
  \inheritanchor[from=rectangle]{north west}
  \inheritanchor[from=rectangle]{north east}
  \inheritanchor[from=rectangle]{center}
  \inheritanchor[from=rectangle]{west}
  \inheritanchor[from=rectangle]{east}
  \inheritanchor[from=rectangle]{mid}
  \inheritanchor[from=rectangle]{mid west}
  \inheritanchor[from=rectangle]{mid east}
  \inheritanchor[from=rectangle]{base}
  \inheritanchor[from=rectangle]{base west}
  \inheritanchor[from=rectangle]{base east}
  \inheritanchor[from=rectangle]{south}
  \inheritanchor[from=rectangle]{south west}
  \inheritanchor[from=rectangle]{south east}
  \inheritanchorborder[from=rectangle]
  \backgroundpath{
    \southwest \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgfpathmoveto{\pgfqpoint{\pgf@xa}{\pgf@yb}}
    \pgfpathlineto{\pgfqpoint{\pgf@xb}{\pgf@ya}}
  }
  \foregroundpath{
    \southwest \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgfpathmoveto{\pgfqpoint{\pgf@xa}{\pgf@ya}}
    \pgfpathlineto{\pgfqpoint{\pgf@xb}{\pgf@yb}}
 }
}
\pgfdeclareshape{knot vert}
{
  \inheritsavedanchors[from=rectangle] % this is nearly a circle
  \inheritanchorborder[from=rectangle]
  \inheritanchor[from=rectangle]{north}
  \inheritanchor[from=rectangle]{north west}
  \inheritanchor[from=rectangle]{north east}
  \inheritanchor[from=rectangle]{center}
  \inheritanchor[from=rectangle]{west}
  \inheritanchor[from=rectangle]{east}
  \inheritanchor[from=rectangle]{mid}
  \inheritanchor[from=rectangle]{mid west}
  \inheritanchor[from=rectangle]{mid east}
  \inheritanchor[from=rectangle]{base}
  \inheritanchor[from=rectangle]{base west}
  \inheritanchor[from=rectangle]{base east}
  \inheritanchor[from=rectangle]{south}
  \inheritanchor[from=rectangle]{south west}
  \inheritanchor[from=rectangle]{south east}
  \inheritanchorborder[from=rectangle]
  \backgroundpath{
    \southwest \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgfpathmoveto{\pgfqpoint{\pgf@xa}{\pgf@ya}}
    \pgfpathlineto{\pgfqpoint{\pgf@xa}{\pgf@yb}}
    \pgfpathmoveto{\pgfqpoint{\pgf@xb}{\pgf@yb}}
    \pgfpathlineto{\pgfqpoint{\pgf@xb}{\pgf@ya}}
 }
}
\pgfdeclareshape{knot horiz}
{
  \inheritsavedanchors[from=rectangle] % this is nearly a circle
  \inheritanchorborder[from=rectangle]
  \inheritanchor[from=rectangle]{north}
  \inheritanchor[from=rectangle]{north west}
  \inheritanchor[from=rectangle]{north east}
  \inheritanchor[from=rectangle]{center}
  \inheritanchor[from=rectangle]{west}
  \inheritanchor[from=rectangle]{east}
  \inheritanchor[from=rectangle]{mid}
  \inheritanchor[from=rectangle]{mid west}
  \inheritanchor[from=rectangle]{mid east}
  \inheritanchor[from=rectangle]{base}
  \inheritanchor[from=rectangle]{base west}
  \inheritanchor[from=rectangle]{base east}
  \inheritanchor[from=rectangle]{south}
  \inheritanchor[from=rectangle]{south west}
  \inheritanchor[from=rectangle]{south east}
  \inheritanchorborder[from=rectangle]
  \foregroundpath{
    \southwest \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgfpathmoveto{\pgfqpoint{\pgf@xa}{\pgf@ya}}
    \pgfpathlineto{\pgfqpoint{\pgf@xb}{\pgf@ya}}
    \pgfpathmoveto{\pgfqpoint{\pgf@xa}{\pgf@yb}}
    \pgfpathlineto{\pgfqpoint{\pgf@xb}{\pgf@yb}}
 }
}
%% 
%% Copyright (C) 2011 by Andrew Stacey <stacey@math.ntnu.no>
%% 
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License (LPPL), either
%% version 1.3c of this license or (at your option) any later
%% version.  The latest version of this license is in the file:
%% 
%% http://www.latex-project.org/lppl.txt
%% 
%% This work is "maintained" (as per LPPL maintenance status) by
%% Andrew Stacey.
%% 
%% This work consists of the files  spath3.dtx
%%                                  calligraphy_doc.tex
%%                                  knot_doc.tex
%% and the derived files            spath3.ins,
%%                                  spath3.pdf,
%%                                  spath3.sty,
%%                                  tikzlibrarycalligraphy.code.tex
%%                                  tikzlibraryknots.code.tex
%%                                  calligraphy_doc.pdf
%%                                  knots_doc.pdf
%%                                  README.txt
%% 
%%
%% End of file `tikzlibraryknots.code.tex'.

